Analysis and improvement of a semi-Lagrangian exponential scheme for the shallow-water equations on the rotating sphere

In this work, we study and extend a class of semi-Lagrangian exponential methods, which combine exponential time integration techniques, suitable for integrating stiff linear terms, with a semi-Lagrangian treatment of nonlinear advection terms. Partial differential equations involving both processes arise for instance in atmospheric circulation models. Through a truncation error analysis, we show that previously formulated semi-Lagrangian exponential schemes are limited to first-order accuracy due to the approximation of the integration factor acting on the discretization of the linear term; we then formulate a new discretization leading to second-order accuracy. Also, a detailed stability study is conducted to compare several Eulerian and semi-Lagrangian exponential schemes, as well as a well-established semi-Lagrangian semi-implicit method, which is used in operational atmospheric models. Numerical simulations of the shallow-water equations on the rotating sphere are performed to assess the orders of convergence, stability properties, and computational cost of each method. The proposed second-order semi-Lagrangian exponential method was shown to be more stable and accurate than the previously formulated schemes of the same class at the expense of larger wall-clock times; however, the method is more stable and has a similar cost compared to the well-established semi-Lagrangian semi-implicit method; therefore, it is a competitive candidate for potential operational applications in atmospheric circulation modeling.

==> alternative_SLETD2RK/new_method.tex <==
\indent The truncation error analysis presented above indicates that the approximation of the linear term is responsible for the first-order accuracy of the \SE{1}{2} scheme. Therefore, we provide an alternative formulation for this approximation which is effectively a second-order one. Consider first the PDE \eqref{eq:base_equation_slexp}, in the Lagrangian framework, with only the linear and (non-linear) advective terms:

\begin{equation}
    \label{eq:base_equation_slexp_linear}
    \frac{\xDif{\vecU}}{\xDif{t}} = \vecL \vecU, \qquad \vecU(t = 0) = \vecU_0,
\end{equation}

\noindent whose solution reads

\begin{equation}
    \label{eq:exact_solution_slexp_linear}
    \vecU(t_{n+1}, \vecx(t_{n+1})) = P_n^{-1}(t_{n+1})\vecU(t_n, \vecx(t_n)), \qquad P_n(t) = e^{-\int_{t_n}^t \vecL_{\vecx(s)}ds}.
\end{equation}

\noindent under the assumptions on $P_n$ and $\vecL_{\vecx(s)}$ described in Section \ref{subsec:sletdrk}. In the \SE{1}{1} and \SE{1}{2} schemes, the integral in $P_{n}(t_{n+1})$ is approximated by considering a constant value $\vecL_{\vecx(s)} = \vecL_{\vecx(t_{n+1})}$ in $[t_n, t_{n+1}]$ along each Lagrangian trajectory $(t,\vecx(t))$, such that \eqref{eq:exact_solution_slexp_linear} reads

\begin{equation}
    \label{eq:exact_solution_slexp_linear_constant}
    \vecU(t_{n+1}, \vecx(t_{n+1})) = e^{\Dt \vecL_{\vecx(t_{n+1})}}\vecU(t_n, \vecx(t_n)) = e^{\Dt \vecL_{\vecx(t_{n+1})}} \vecU^n_*
\end{equation}

\noindent which can be interpreted as follows: the solution is obtained at $t_{n+1}$ through interpolation, then the linear operator, also evaluated at $t_{n+1}$, is applied to it.

\indent We propose to approximate the integral in the integration factor considering a trapezoidal rule:

\begin{equation}
    \label{eq:trapezoidal}
    \added[id=R1]{P_n(t_{n+1}) \approx e^{-\frac{\Dt}{2} \left[\vecL_{\vecx(t_{n+1})} + \vecL_{\vecx(t_{n})}\right]}}
\end{equation}


\noindent such that \eqref{eq:exact_solution_slexp_linear} reads

% \begin{equation}
%     \label{eq:exact_solution_slexp_linear_trapezoidal}
%     \vecU(t_{n+1}, \vecx(t_{n+1})) = e^{\frac{\Dt}{2} \vecL_{\vecx(t_{n+1})}} \left[ e^{\frac{\Dt}{2} \vecL_{\vecx(t_{n})}} \vecU(t_n, \vecx(t_n))\right](t_n, \vecx(t_n)) = e^{\frac{\Dt}{2} \vecL_{\vecx(t_{n+1})}} \left[ e^{\frac{\Dt}{2} \vecL_{\vecx(t_{n})}} \vecU\right]^n_*
% \end{equation}

%suggestion
\begin{equation}
    \label{eq:exact_solution_slexp_linear_trapezoidal}
    \vecU(t_{n+1}, \vecx(t_{n+1})) = e^{\frac{\Dt}{2} \vecL_{\vecx(t_{n+1})}} \left[ e^{\frac{\Dt}{2} \vecL_{\vecx(t_{n})}} \vecU(t_n, \vecx(t_n))\right]_{(t_n, \vecx(t_n))} = e^{\frac{\Dt}{2} \vecL_{\vecx(t_{n+1})}} \left[ e^{\frac{\Dt}{2} \vecL_{\vecx(t_{n})}} \vecU\right]^n_*
\end{equation}


\noindent \ie following the same interpretation as in \eqref{eq:exact_solution_slexp_linear_constant}, half of the linear operator, evaluated at $t_n$, is applied to the solution computed at $t_n$; then the solution is obtained at $t_{n+1}$ through interpolation; finally, half of the linear operator at $t_{n+1}$ is applied to the solution. This interpretation suggests relatively straightforward ways to derive higher-order semi-Lagrangian exponential discretizations of the linear term, by considering higher-order approximations of the integral, \eg the Simpson's rule, in which case additional difficulties concerning the evaluation of $\vecL_{\vecx(s)}$ at intermediate points of the Lagrangian trajectories would need to be dealt with.

\indent As shown both analytically and numerically in the next sections, \eqref{eq:exact_solution_slexp_linear_trapezoidal} is a second-order discretization of the linear term. \replaced[id=R1]{Applying it to the full PDE \eqref{eq:base_equation_exp}}{Applying it to the full PDE \eqref{eq:pde_SL}}, we obtain the methods:

\begin{subequations}
    \begin{align}
    \vecU^{n+1}_{\text{\SE{2}{1}}} &=  \varphi_0\left(\frac{\Dt L}{2}\right) \left[ \varphi_0\left(\frac{\Dt L}{2}\right) \vecU^n \right]^n_* +   \varphi_0(\Dt L) \left[\Dt \psi_1(\Dt L) \tilde{\vecN}(\vecU^n) \right]_*^n, \label{eq:SL-ETD1RK-new}\\
    \vecU^{n+1}_{\text{\SE{2}{2}}} &=  \vecU^{n+1}_{\text{\SE{2}{1}}} + \Dt \varphi_0(\Dt L ) \left[\psi_2(\Dt L) \tilde{\vecN}(\vecU^{n+1}_{\text{\SE{2}{1}}}) - \left( \psi_2(\Dt L) \tilde{\vecN} (\vecU^n)        \right)^n_* \right]. \label{eq:SL-ETD2RK-new}
    \end{align}
\end{subequations}

\noindent \added[id=R1]{where the Lagrangian trajectories are estimated as in the \SE{1}{1} and \SE{1}{2} schemes, using SETTLS (Eq. \eqref{eq:SETTLS}).}

\indent The names of the methods were chosen following the same reasoning as before. In \eqref{eq:SL-ETD1RK-new}, a second- and a first-order discretizations of the linear and nonlinear terms, respectively, resulting in a global first-order approximation; in \eqref{eq:SL-ETD2RK-new}, a global second-order accuracy is ensured by second-order discretizations of both linear and nonlinear terms. 

\indent Note that the proposed discretization, using the approximation \eqref{eq:trapezoidal} to the integration factor, is applied only to the linear term, \ie the nonlinear one is discretized as in \SE{1}{1} (eq. \eqref{eq:ETD1RK}) and \SE{1}{2} (eq. \eqref{eq:ETD2RK}). As verified in the numerical experiments in Section \ref{sec:numerical_simulations}, the discretization of the nonlinear term proposed by \cite{peixoto_schreiber:2019} in \SE{1}{2} has second-order accuracy, such that \SE{2}{2} achieves second-order with a relatively simple approximation of the exponential functions; the application of \eqref{eq:trapezoidal} to the nonlinear term would lead to a much more complex formulation, since the integration factor acts both inside and outside the integral in \eqref{eq:exact_solution_slexp}.

\indent In the following paragraphs, we prove analytically the second-order convergence of the proposed discretization considering only the linear term. In order to provide a more complete comparative study with the original formulation of the SL-ETDRK schemes, as well as with SL-SI-SETTLS and the Eulerian ETDRK methods, we also present an estimate of the computing complexity and, in Section \ref{subsec:serial_stability}, a detailed linear stability analysis. In Section \ref{sec:numerical_simulations}, we provide a numerical verification of these aspects considering the full nonlinear SWE on the rotating sphere.
% \deleted[id=MS]{which shows that the proposed modification, combined with the discretization for the nonlinear term proposed by \cite{peixoto_schreiber:2019}, results in a second-order semi-Lagrangian exponential scheme for the SWE on the rotating sphere.}

\indent It is worth noting that linear and interpolation operators do not commute in general (see Appendix of \cite{peixoto_schreiber:2019}), such that, even with $\varphi_0(\Dt L /2) \varphi_0(\Dt L /2) = \varphi_0(\Dt L)$, we may have

\begin{equation}
    \label{eq:commutation}
    \varphi_0(\Dt L)[\vecU^n]^n_* \neq \varphi_0\left(\frac{\Dt L}{2}\right)\left[\varphi_0\left(\frac{\Dt L}{2}\right) \vecU^n\right]^n_* .
\end{equation}

\indent Finally, we highlight the similarities and differences of the proposed method \wrt the semi-Lagrangian Rosenbrock-type exponential schemes proposed by \cite{shashkin_goyman:2020}. In both methods, a splitting of the time step integration is performed in order to achieve second-order accuracy. In \cite{shashkin_goyman:2020}, this is made by evolving the fluid particles along the Lagrangian trajectory from $t_n$ to $t_{n+1/2} := t_n + \Dt/2$, applying the exponential operator at $t_{n+1/2}$, and evolving the fluid particles from $t_{n+1/2}$ to $t_n$. Here, we consider a different splitting, with two applications of the exponential operator and a single application of the semi-Lagrangian approach; also, both applications of the exponential operator are identical, corresponding to a left multiplication by the constant matrix $\varphi_0(\Dt L/2)$. Moreover, as described in Section \ref{subsec:ETDRK}, we consider a spectral discretization in space, which, with a proper rearrangement of the terms of the governing equations, allows for a straightforward computation of the matrix exponentials, while these are approximated in \cite{shashkin_goyman:2020} using Krylov-subspace methods.

==> alternative_SLETD2RK/truncation_error.tex <==
\subsection{Truncation error analysis}

\indent We conduct a similar reasoning as before to compute the truncation error of the scheme

\begin{equation}
    \label{eq:linear_SLETD2RK_v2}
    U^{n+1} = \varphi_0 \left( \frac{\Dt L}{2} \right) \left[\varphi_0 \left( \frac{\Dt L}{2} \right) U^n \right]^n_*
\end{equation}

\noindent approximating Eq. \eqref{eq:PDE}. Three steps can be identified in this approximation: (i) evolution along the trajectory from $(t_n, x_d)$ to the midpoint $(t_{n+1/2}, x_m)$; (ii) interpolation of the computed solution to the midpoint; (iii) evolution along the trajectory from $(t_{n+1/2}, x_m)$ to $(t_{n+1}, x_j)$. Therefore, the truncation error can be written as

% \begin{equation}
\begingroup
\allowdisplaybreaks
    \begin{align}
        \tau_j^{n+1} && = & \frac{1}{\Dt} \left[ u^{n+1}_j - \phizerotwo \sum_{k=-r}^q \beta_k \phizerotwo u^n_{j-p+k}\right] = \underbrace{\frac{1}{\Dt} \left[ u^{n+1}_j - \phizerotwo u^{n+1/2}_m \right]}_{(\tau_j^{n+1})_1} +\notag\\
        && & \underbrace{\frac{1}{\Dt} \left[ \phizerotwo u^{n+1/2}_m - \phizerotwo \sum_{k=-r}^q \beta_k u^{n+1/2}_{j-\tilde{p}+k} \right]}_{(\tau_j^{n+1})_2} + \notag\\
        && & \underbrace{\frac{1}{\Dt} \left[ \phizerotwo \sum_{k=-r}^q \beta_k u^{n+1/2}_{j-\tilde{p}+k} - \phizerotwo \sum_{k=-r}^q \beta_k \phizerotwo u^n_{j-p+k} \right]}_{(\tau_j^{n+1})_3}\label{eq:truncation_error_V2}
    \end{align}
\endgroup
% \end{equation}

\noindent where $j - \tilde{p}$ is the index of the closest grid point to the right of $x_m$ (see Figure \ref{fig:lagrangian_trajectory}). Since the trajectory is considered to be linear in the SETTLS approximation, $x_m$ satisfies $x_j - x_m = s/2 = \Dt V^{n+1/2}_m/2$.


\indent The first term in \eqref{eq:truncation_error_V2} ($(\tau^{n+1}_j)_1$) accounts for the error in the estimation of the point $x_m$; the second term ($(\tau^{n+1}_j)_2$) accounts for the interpolation error, and the last term ($(\tau^{n+1}_j)_3$) accounts for the error in the estimation of $x_d$. 
The second term is completely analogous to \eqref{eq:interpolation_error}, so it is $\mc{O}(\Dx^3/\Dt)$. 

% \begin{figure}[!htbp]
%     \centering
%     \includegraphics{alternative_SLETD2RK/figures/TikZfigures-truncation_error_SLETDRK_V2.pdf}
%     \caption{Lagrangian trajectory in $[t_n, t_{n+1}]$}
%     \label{fig:lagrangian_trajectory_V2}
% \end{figure}

\indent The first term in \eqref{eq:truncation_error_V2} reads

\begingroup
\allowdisplaybreaks
% \begin{equation}
    \begin{align}
        (\tau_j^{n+1})_1 && = \frac{1}{\Dt} & \left[ u^{n+1}_j - \phizerotwo u_m^{n+1/2}\right] \notag\\
        && = \frac{1}{\Dt} & \left[ u^{n+1/2}_m + \frac{\Dt}{2} u_t|_m^{n+1/2} + \frac{s}{2} u_x|_m^{n+1/2} + \right. \notag\\
        && & + \frac{\Dt^2}{8} u_{tt}|_m^{n+1/2} + \frac{\Dt s}{4} u_{tx}|_m^{n+1/2} + \frac{s^2}{8} u_{xx}|_m^{n+1/2} + \mc{O}(\Dt^3) + \mc{O}(s^3) \notag\\
        && & \left. - \left( 1 + \frac{\Dt L}{2} + \frac{\Dt^2L^2}{8} + \mc{O}(\Dt^3) \right) u_m^{n+1/2}\right] \notag\\
        && = \frac{1}{\Dt} & \left[ \frac{\Dt}{2}\left(u_t|_m^{n+1/2} + vu_x|_m^{n+1/2} - Lu_m^{n+1/2}\right) \right. \notag\\
        && & \left. + \frac{\Dt^2}{8} \left( u_{tt}|_m^{n+1/2} + 2 (v u)|_m^{n+1/2}  + (v^2u_{xx})|_m^{n+1/2} - L^2u_m^{n+1/2} \right) + \mc{O}(\Dt^3)  \right] \notag\\
        && = \frac{1}{\Dt} & \left[ \frac{\Dt^2}{8} \left( u_{tt}|_m^{n+1/2} + 2 (v u)|_m^{n+1/2}  + (v^2u_{xx})|_m^{n+1/2} - L^2u_m^{n+1/2} \right) + \mc{O}(\Dt^3)  \right] \label{eq:truncation_error_new_1}
    \end{align}
% \end{equation}
\endgroup

\noindent where we used the facts that $Lu = u_t + vu_x$ and

\begin{equation}
    \label{eq:truncation_error_new_s}
    s = x_j - x_d = \frac{\Dt}{2} \left( 2v(t_n,x_d) - v(t_{n-1},x_d) + v(t_n, x_j) \right) = \Dt v_m^{n+1/2} + \mc{O}(\Dt^3)
\end{equation}

\noindent For computing the last term in \eqref{eq:truncation_error_V2}, we note that, from \eqref{eq:interpolation_error}, the cubic interpolation yields

\begin{equation}
    \label{eq:truncation_error_new_interpolation}
    \sum_{k=-r}^q{\beta_k w_{j-p+k}} = w_d + \mc{O}(\Dx^3), \qquad \sum_{k=-r}^q{\beta_k w_{j-\tilde{p}+k}} = w_m + \mc{O}(\Dx^3)
\end{equation}

\noindent for every function $w = w(x)$. Therefore,

\begingroup
\allowdisplaybreaks
% \begin{equation}
    \begin{align}
        \left(\tau_j^{n+1}\right)_3 && = \frac{1}{\Dt} & \left[ \phizerotwo \sum_{k=-r}^q \beta_k u^{n+1/2}_{j-\tilde{p}+k} - \phizerotwo\sum_{k=-r}^q \beta_k \phizerotwo u^n_{j-p+k} \right] \notag\\
        &&  = \frac{1}{\Delta t}  & \phizerotwo  \left[ u^{n+1/2}_m - \phizerotwo u^n_d + \mc{O}(\Dx^3) \right] \notag\\
        && = \frac{1}{\Dt}  &\left( 1 + \frac{\Dt L}{2} + \frac{\Dt^2 L^2}{8} + \mc{O}(\Dt^3) \right)  \left[ u^{n+1/2}_m - \left( 1 + \frac{\Dt L}{2} +  \frac{\Dt^2 L^2}{8} + \mc{O}(\Dt^3) \right) \right. \notag\\
        && & \left. \left( u^{n+1/2}_m - \frac{\Dt}{2}u_t|_m^{n+1/2} - \frac{s}{2}u_x|_m^{n+1/2} \right. \right.\notag\\
        && & \left. \left.+  \frac{\Dt^2}{8}u_{tt}|_d^{n+1/2} +  \frac{\Dt s}{4}u_{tx}|_d^{n+1/2} +  \frac{s^2}{8}u_{xx}|_d^{n+1/2} + \mc{O}(\Dt^3)\right) + \mc{O}(\Dx^3)\right] \notag\\
        && = \frac{1}{\Dt} & \left[  \frac{\Dt}{2} \left(-Lu_m^{n+1/2} + u_t|_m^{n+1/2} + (vu_x)|_m^{n+1/2}\right) \right. \notag\\
        && & \left. + \frac{\Dt^2}{8} \left( -3L^2u_m^{n+1/2} + 4Lu_t|_m^{n+1/2} + 2L(vu_x)|_m^{n+1/2} \right. \right.\notag\\
        && & \left. \left. - u_{tt}|_m^{n+1/2} - 2(vu_{tx})|_m^{n+1/2} - (v^2u_{xx})|_m^{n+1/2}
 \right) + \mc{O}(\Dt^3) + \mc{O}(\Dx^3)   \right] \notag\\
       && =  \frac{1}{\Dt} & \left[ \frac{\Dt^2}{8} \left( -3L^2u_m^{n+1/2} + 4Lu_t|_m^{n+1/2} + 2L(vu_x)|_m^{n+1/2} \right. \right. \notag\\
       && & \left. \left. - u_{tt}|_m^{n+1/2} - 2(vu_{tx})|_m^{n+1/2} - (v^2u_{xx})|_m^{n+1/2}
 \right) \right. \notag\\
        && & \left. + \mc{O}(\Dt^3) + \mc{O}(\Dx^3)  \right] \label{eq:truncation_error_new_3}
    \end{align}
% \end{equation}
\endgroup

\noindent Adding the three terms in \eqref{eq:truncation_error_V2}, we get

\begin{equation}
    \label{eq:truncation_error_new}
    \begin{aligned}
        \tau_j^{n+1} & = \frac{1}{\Dt} \left[ \frac{4\Dt^2L}{8} \left( -Lu_m^{n+1/2} + u_t|_m^{n+1/2} + (vu_x)|_m^{n+1/2} \right)  \right] + \mc{O}(\Dt^2) + \mc{O}\left(\frac{\Dx^3}{\Dt}\right)\\
        & = \mc{O}(\Dt^2)
    \end{aligned}
\end{equation}

\noindent thus yielding a second-order approximation.

